Towards Quantifying Neurovascular Resilience

Whilst grading neurovascular abnormalities is critical for prompt surgical repair, no statistical markers are currently available for predicting the risk of adverse events, such as stroke, and the overall resilience of a network to vascular complications. The lack of compact, fast, and scalable simulations with network perturbations impedes the analysis of the vascular resilience to life-threatening conditions, surgical interventions and long-term follow-up. We introduce a graph-based approach for efficient simulations, which statistically estimates biomarkers from a series of perturbations on the patient-specific vascular network. Analog-equivalent circuits are derived from clinical angiographies. Vascular graphs embed mechanical attributes modelling the impedance of a tubular structure with stenosis, tortuosity and complete occlusions. We evaluate pressure and flow distributions, simulating healthy topologies and abnormal variants with perturbations in key pathological scenarios. These describe the intrinsic network resilience to pathology, and delineate the underlying cerebrovascular autoregulation mechanisms. Lastly, a putative graph sampling strategy is devised on the same formulation, to support the topological inference of uncertain neurovascular graphs.

==> [CVII-STENT] Towards Quantifying Neurovascular Resilience/references.tex <==
\begin{thebibliography}{10}

\bibitem{VMTK2008}
L.~Antiga and D.~Steinman.
\newblock {The Vascular Modeling Toolkit}, 2008.

\bibitem{aylward2012tubetk}
S.~Aylward, et al.
\newblock {TubeTK, Segmentation, Registration, and Analysis of Tubular
  Structures in Images}.
\newblock {\em Kitware Inc.}, 2012.

\bibitem{cebral2005characterization}
J.~R. Cebral, et al.
\newblock Characterization of cerebral aneurysms for assessing risk of rupture
  by using patient-specific computational hemodynamics models.
\newblock {\em Am J Neuroradiol}, 2005.

\bibitem{cheng2015accurate}
Y.~Cheng, et al.
\newblock Accurate vessel segmentation with constrained b-snake.
\newblock {\em IEEE Trans Image Process}, 2015.

\bibitem{chnafa2017improved}
C.~Chnafa, et al.
\newblock Improved reduced-order modelling of cerebrovascular flow distribution
  by accounting for arterial bifurcation pressure drops.
\newblock {\em J Biomech}, 2017.

\bibitem{fossan2018optimization}
F.~E. Fossan, et al.
\newblock Optimization of topological complexity for one-dimensional arterial
  blood flow models.
\newblock {\em J Royal Soc Interface}, 2018.

\bibitem{mathers2008global}
C.~Mathers, et al.
\newblock {\em {The Global Burden of Disease: 2004 Update}}.
\newblock World Health Organization, 2008.

\bibitem{moriconi2018inference}
S.~Moriconi, et al.
\newblock Inference of cerebrovascular topology with geodesic minimum spanning
  trees.
\newblock {\em IEEE TMI}, 2018.

\bibitem{onaizah2017model}
O.~Onaizah, et al.
\newblock A model of blood supply to the brain via the carotid arteries:
  Effects of obstructive vs. sclerotic changes.
\newblock {\em Med Eng Phys}, 2017.

\bibitem{ryu2015coupled}
J.~Ryu, et al.
\newblock A coupled lumped-parameter and distributed network model for cerebral
  pulse-wave hemodynamics.
\newblock {\em J Biomech Eng}, 2015.

\bibitem{shojima2004magnitude}
M.~Shojima, et al.
\newblock Magnitude and role of wall shear stress on cerebral aneurysm:
  computational fluid dynamic study of 20 MCA aneurysms.
\newblock {\em Stroke}, 2004.

\bibitem{steinman2003computational}
D.~Steinman, et al.
\newblock Computational modeling of arterial biomechanics: Insights into
  pathogenesis and treatment of vascular disease.
\newblock {\em J Vasc Surg}, 2003.

\bibitem{taylor2009open}
C.~Taylor and J.~Humphrey.
\newblock Open problems in computational vascular biomechanics: Hemodynamics
  and arterial wall mechanics.
\newblock {\em CMAME}, 2009.

\bibitem{urick2017review}
B.~Urick, et al.
\newblock Review of patient-specific vascular modeling: template-based
  isogeometric framework and the case for cad.
\newblock {\em Arch Comput Methods Eng}, 2017.

\bibitem{vitturi2016navier}
M.~D. Vitturi.
\newblock Navier-stokes equations in cylindrical coordinates, 2016.

\end{thebibliography}

